Mid-Infrared Detectors and Imagers Integrating All-Group IV Nanowires

Cost-effective mid-wave infrared (MWIR) optoelectronic devices are of utmost importance to a plethora of applications such as night vision, thermal sensing, autonomous vehicles, free-space communication, and spectroscopy. To this end, leveraging the ubiquitous silicon-based processing has emerged as a powerful strategy that can be accomplished through the use of group IV germanium-tin (GeSn) alloys. Indeed, due to their compatibility with silicon and their tunable bandgap energy covering the entire MWIR range, GeSn semiconductors are frontrunner platforms for compact and scalable MWIR technologies. However, the GeSn large lattice parameter has been a major hurdle limiting the quality of GeSn epitaxy on silicon wafers. Herein, it is shown that sub-20 nm Ge nanowires (NWs) provide effective compliant substrates to grow Ge$_{1-x}$Sn$_{x}$ alloys with a composition uniformity over several micrometers with a very limited build-up of the compressive strain. Ge/Ge$_{1-x}$Sn$_{x}$ core/shell NWs with Sn content spanning the 6 to 18 at.$\%$ range are demonstrated and integrated in photoconductive devices exhibiting a high signal-to-noise ratio at room temperature and a tunable cutoff wavelength covering the 2.0 $\mu$m to 3.9 $\mu$m range. Additionally, the processed NW-based detectors were used in uncooled imagers enabling the acquisition of high-quality images under both broadband and laser illuminations without a lock-in technique.

==> utils/space_saving_tricks.tex <==
%% Make everything look better.
%% http://tex.stackexchange.com/questions/553/what-packages-do-people-load-by-default-in-latex
%% http://www.howtotex.com/packages/9-essential-latex-packages-everyone-should-use/
\usepackage{microtype}

%% Shrink space around figures.
%% This beats manually adding negative \vspace commands everywhere.
\setlength{\textfloatsep}{0pt}
\setlength{\textfloatsep}{20pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{10pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{10pt plus 1pt minus 2pt}
\setlength{\dbltextfloatsep}{3pt}
\setlength{\intextsep}{5pt}
\setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{3pt}
\setlength{\parskip}{4pt}
%% around equations
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\setlength\abovedisplayshortskip{3pt}
\setlength\belowdisplayshortskip{3pt}


%% The wrapfigure environment is also a good way to use less space for a small figure.
%% It is finicky.
%% See: http://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Wrapping_text_around_figures

%% Shrink space around enumerate and itemize
%% From: http://tex.stackexchange.com/questions/10684/vertical-space-in-lists
\usepackage{enumitem}
%% Set it globally:
\setlist{nosep} % or \setlist{noitemsep} to leave space around whole list
\setlist{itemsep=1pt, topsep=3pt}
%% Or locally:
% \begin{enumerate}[itemsep=1pt, topsep=12pt, partopsep=0pt]

%% Less space around titles.
%% From: http://tex.stackexchange.com/questions/4999/change-whitespace-above-and-below-a-section-heading
%\usepackage[medium,compact]{titlesec}
%% or
%\usepackage{titlesec}
%\titlespacing*{\section}{0pt}{*1}{*1}

%% Shrink the \paragraph command.
\renewcommand{\paragraph}[1]{\noindent {\bf #1}}

%% Allow Latex to use a smaller minimum spacing between lines.
%\renewcommand{\baselinestretch}{0.97}
%\renewcommand{\baselinestretch}{0.982}

%% Shrink space between lines. You probably want to prefer baselinestretch in general.
%% From: http://tex.stackexchange.com/questions/23824/6-lines-in-one-inch
%% 6 lines in one inch with an 11pt font:
%\linespread{0.901}
%\linespread{0.909}
%\linespread{1}

%% Shrink the spacing between lines in just the bibliography. This is good.
\usepackage{setspace}

%% Then wrap the bibliography in a \begin{spacing}. You can wrap any section like this.
% \begin{spacing}{0.9}
% \bibliographystyle{...}
% \bibliography{references}
% \end{spacing}
